Extensional concepts in intensional type theory, revisited

Revisiting a classic result from M. Hofmann's dissertation, we give a direct proof of Morita equivalence, in the sense of V. Isaev, between extensional type theory and intensional type theory extended by the principles of functional extensionality and of uniqueness of identity proofs.

==> cofib.tex <==
\section{Classification of Types in Cofibrant Models}
%
A key step in Hoffman's original proof in the syntactic setting was the ability
to define maps between contexts based on the outer-most type former of the last
type in context.
%
Although our definition of Morita equivalence in \Cref{def:morita} defines a
Morita equivalence between two theories as a Quillen adjunction between the
categories of their models whose units at cofibrant models are weak equivalences
and is therefore more general than the syntactic setting, cofibrancy
nevertheless allows one to recover the following syntax-like property of
cofibrant models.
%
Namely, as cofibrant models are obtained by freely adjoining types and terms,
but no judgemental equalities, to the initial model, they have a syntax-like
property that allows one to classify types into the mutually exclusive cases of
$\Pi$-types, $\Id$-types, $\Sigma$-types or base types.
%
This syntax-like property is the key that allows Hoffman's proof to be
reproduced in our more general setting.
%
\begin{proposition}\label{prop:cofib-ty-class}
  %
  If $\bC \in \CxlCat_\ITT$ is a cofibrant model then there is a set
  $\set{(\Theta_i \in \bC, A_i \in \Ty_\bC\Theta_i)}_{i \in I}$ such that each
  object $\Gamma \in \ob_{n+1}\bC$ for $n \in \bN$ is exactly one of the
  following mutually exclusive cases:
  %
  \begin{itemize}
    %
    \item \emph{$\Pi$-types.} $\Gamma = \Delta.\Pi(X,Y)$ for unique
    $\Delta \in \bC$ and $X.Y \in \Ty\Delta$.
    %
    \item \emph{$\Sigma$-types.} $\Gamma = \Delta.\Sigma(X,Y)$ for unique
    $\Delta \in \bC$ and $X,Y \in \Ty\Delta$.
    %
    \item \emph{$\Id$-types.} $\Gamma = \Delta.X.X.\Id_X$ for unique
    $\Delta \in \bC$ and $X \in \Ty\Delta$.
    %
    \item \emph{Base types.} $\Gamma = \Delta.f^*A_i$ for unique
    $\Delta \in \bC$ and $f \colon \Delta \to \Theta_i$ and moreover
    $\Gamma \neq \Delta.g^*A_i$ for any $g \colon \Delta \to \Theta_j$ where
    $j \neq i$.
    %
  \end{itemize}
  %
  Moreover, there is a well-founded order $<$ on $\ob\bC$ such that:
  %
  \begin{align*}
    \Gamma.X.Y < \Gamma.\Pi(X,Y), \Gamma.\Sigma(X,Y)
    &&
       \Gamma < \Gamma.X
       \qedhere
  \end{align*}
  %
\end{proposition}

Intuitively, this result holds because \Cref{def:ctx-cofib} defines the
cofibrant models as those obtained by repeatedly freely adjoining base types and
terms, but no definitional equalities, starting from the initial model, which is
simply the model consisting of just the empty context.
%
In each step when a base type is freely adjoined, $\Pi$-, $\Id$- and
$\Sigma$-types that can be obtained using combinations of this new base type are
also formally added.
%
In what follows, we formalise this intuition.
%
The key lies in giving an explicit description of the $\CwA$ obtained from
freely adjoining a type or term to a given $\CwA$.

\iffalse

The proof of this result relies on cofibrant models having a presentation as an
$\McI$-cell complex as in \Cref{def:ctx-cofib}.
%
Indeed, pushing out along
$\vvbr{\Ctx_n} \hookrightarrow \vvbr{\Ctx_n \vdash \Type}$ amounts to freely
adjoining a new type in a context of length $n$, while pushing out along
$\vvbr{\Ctx_n \vdash \Type} \hookrightarrow \vvbr{\Ctx_n \vdash \Term : \Type}$
amounts to freely adjoining a term of a specified type in a context of length
$n$.
%
In both cases, no new definitional equalities are added.
%
\TODO{Revise presentation of \Cref{prop:cofib-ty-class}.}


Hofmann's original proof was done in the setting of the syntactic category of
$\ITT$ and relied heavily on discussion by cases based on the outer-most
type-former of types.
%
In the general setting of arbitrary contextual categories however, one may have
equalities between types, such as $\Pi(A,B) = \Sigma(A,B)$.
%
Fortunately, however, when we limit ourselves to the \emph{cofibrant} models,
such equalities are impossible and we recover a classification property of types
based on their outer-most type formers.
%
In particular, cofibrant models have the following syntax-like property:

\begin{proposition}\label{prop:cofib-ty-class}
  %
  If $\bC \in \CxlCat_\ITT$ is a cofibrant model then there is a set
  $\set{(\Theta_i \in \bC, A_i \in \Ty_\bC\Theta_i)}_{i \in I}$ such that each
  object $\Gamma \in \ob_{n+1}\bC$ for $n \in \bN$ is exactly one of the
  following mutually exclusive cases:
  %
  \begin{itemize}
    %
    \item \emph{$\Pi$-types.} $\Gamma = \Delta.\Pi(X,Y)$ for unique $\Delta \in \bC$ and $X.Y \in \Ty\Delta$.
    %
    \item \emph{$\Sigma$-types.} $\Gamma = \Delta.\Sigma(X,Y)$ for unique
    $\Delta \in \bC$ and $X,Y \in \Ty\Delta$.
    %
    \item \emph{$\Id$-types.} $\Gamma = \Delta.X.X.\Id_X$ for unique $\Delta \in \bC$ and $X \in \Ty\Delta$.
    %
    \item \emph{Base types.} $\Gamma = \Delta.f^*A_i$ for unique
    $\Delta \in \bC$ and $f \colon \Delta \to \Theta_i$ and moreover
    $\Gamma \neq \Delta.g^*A_i$ for any $g \colon \Delta \to \Theta_j$ where
    $j \neq i$.
    %
  \end{itemize}
  %
  Moreover, there is a well-founded order $<$ on $\ob\bC$ such that:
  %
  \begin{align*}
    \Gamma.X.Y < \Gamma.\Pi(X,Y), \Gamma.\Sigma(X,Y)
    &&
       \Gamma < \Gamma.X
       \qedhere
  \end{align*}
  %
\end{proposition}
%
The proof of this result relies on cofibrant models having a presentation as an
$\McI$-cell complex as in \Cref{def:ctx-cofib}.
%
We proceed by giving an explicit description of pushouts in $\CxlCat_\ITT$ along
maps in $\McI$.

We start by examining models of $\ITT$ obtained by freely adjoining a type $T$
in a specified context $\Theta$ of length $n$ to a model $\bC$.
%
Conceptually, freely adjoining a type consists of formally adding a context
$\Theta.T$ to $\bC$, then closing the new category under substitution and
logical constructions.
%
But $\vvbr{\Ctx_n \vdash \Type}$ and $\bC$ are already both closed under
substitution and logical constructions.
%
So what remains is to identify the generator $\Ctx_n$ with $\Theta \in \bC$ and
to close the new category under substitution.
%
This is because logical constructions are stable under substitution, which means
applying logical constructions to substitutions of newly-added types is the same
as applying the logical constructions first before applying substitution.
%
In other words, because $\vvbr{\Ctx_n \vdash \Type}$ is closed under logical
constructions, we may apply the logical constructions in question in this
freely-generated model first and then closing the result under substitution in
$\bC$.
%
Hence, freely adjoining a type $T$ to $\bC$ in context $\Theta \in \bC$ is the
same as adding to $\bC$ formal pullbacks $\Gamma.f^*\vec{X}$ of freely-generated
context extensions $\vec{X}$ of the generic context $\Ctx_n$ of length $n$ by
the generic type $\Type \in \Ty\Ctx_n$ in $\vvbr{\Ctx_n \vdash \Type}$ along
maps $f \colon \Delta \to \Gamma \in \bC$.
%
By noting that each such formal pullback $\Gamma.f^*\vec{X}$ can be expressed as
an object of $\bC/\Theta \times \vvbr{\Ctx_n\vdash\Type}\sslash\Ctx_n$, we are
led to the following definition:
%
\begin{definition}\label{def:free-ty}
  %
  Fix $\bC \in \CxlCat_\ITT$ along with maps $\vvbr{\Ctx_n} \to \bC$ and
  $\vvbr{\Ctx_n} \hookrightarrow \vvbr{\Ctx_n \vdash \Type} \in \McI$.
  %
  Let $\Theta \in \bC$ be the image of the generator $\Ctx_n \in \vvbr{\Ctx_n}$
  under $\vvbr{\Ctx_n} \to \bC$.
  %
  Denote by $\bC \cup_\Theta \Theta.X$ the pushout, in $\Cat$ (as opposed to
  $\CxlCat$):
  %
  \begin{equation*}
    \begin{tikzcd}
      \bC/\Theta \ar[r, "{(\id,\Ctx_n)}"] \ar[d, "\dom{}"']
      \ar[rd, phantom, "\ulcorner"{pos=1}]
      & \bC/\Theta \times \vvbr{\Ctx_n \vdash \Type}\sslash \Ctx_n \ar[d]
      \\
      \bC \ar[r] & \bC \cup_\Theta \Theta.X
    \end{tikzcd} \in \Cat
  \end{equation*}

  We put the structure of a contextual category on $\bC \cup_\Theta \Theta.X$ as
  follows:
  %
  \begin{itemize}
    %
    \item $\ob_m{(\bC \cup_\Theta \Theta.X)}$ consists of either those
    $\Gamma \in \ob_m\bC$ or pairs
    $(f \colon \Gamma \to \Theta \in \bC/\Theta, \vec{X} \in \vvbr{\Ctx_n
      \vdash \Type} \sslash \Ctx_n)$ such that $\Gamma$ is of length $k$ and
    $\vec{X}$ is of length $\ell$ where $k+\ell=m$.
    %
    \item The projection of $\Gamma.A \in \ob_{m+1}\bC$ is given by
    $\pi_A \colon \Gamma.A \to A \in \bC$ and the projection of
    $(f \colon \Gamma \to \Theta \in \bC/\Theta, \vec{X}.S \in
    \vvbr{\Ctx_n \vdash \Type} \sslash \Ctx_n)$ is given by
    $(f \colon \Gamma \to \Theta \in \bC/\Theta, \vec{X} \in \vvbr{\Ctx_n
      \vdash \Type} \sslash \Ctx_n)$, where the first component remains the same
    and the projection happens in the second component.
    %
    \item If $\bC(\Gamma,\Theta) = \emptyset$ then substitution along
    $f \colon \Delta \to \Gamma \in \bC$ is just as it is given in $\bC$.
    %
    Otherwise, substitution along
    %
    \begin{align*}
      (\Delta \xrightarrow{g} \Gamma \xrightarrow{f} \Theta, \vec{X}) \xrightarrow{(g,\id)}
      (\Gamma \xrightarrow{f} \Theta, \vec{X}) \xrightarrow{(\id,t)}
      (\Gamma \xrightarrow{f} \Theta, \vec{S})
      \in \bC/\Theta \times \vvbr{\Ctx_n \vdash \Type} \sslash \Ctx_n
    \end{align*}
    %
    is given by the pullback in
    $\bC/\Theta \times \vvbr{\Ctx_n \vdash \Type} \sslash \Ctx_n$.
    %
  \end{itemize}
  %
\end{definition}

% Following similar reasoning as above, to freely adjoin a term $t$ to a type $T$
% in context $\Theta$ is to freely

\begin{definition}\label{def:syn-pres}
  %
  For each graded set $\McA = \coprod_{n\in\bN}\McA_n$ of axioms in which each
  $\McA_n$ consists of axioms of the form $\Gamma \vdash T~\Type$ and
  $\Gamma \vdash t : T$ where $T \in \McT_n$ and $\Gamma~\Ctx$ is derivable
  using only axioms from $\sqcup_{m<n}\McA_m$, put $\vvbr{\McA}$ to be the
  syntactical category of $\ITT$ extended with axioms of $\McA$.
  %
  A model $\bC \in \CxlCat_\ITT$ is \emph{syntactically presentable} when there is
  some $\McA$ such that $\bC \simeq \vvbr{\McA}$.
  %
  Such a graded set $\McA$ is called the \emph{syntactical presentation} of
  $\bC$.
  %
\end{definition}

\begin{lemma}
  %
  Fix $\McA$ as in \Cref{def:syn-pres}.
  %
  For each $(\vec{x}:\Theta) \colon \vvbr{\Ctx_\ell} \to \McA$, put
  $\McA^{(\vec{x}:\Theta).\MsX(\vec{x})} \coloneqq \McA_n^{(\vec{x}:\Theta).\MsX(\vec{x})}$, where each
  $\McA_n^{(\vec{x}:\Theta).\MsX(\vec{x})} \coloneqq \McA_n$ for $n \neq \ell$ and
  $\McA_\ell^{(\vec{x}:\Theta).\MsX(\vec{x})} \coloneqq \McA_\ell \sqcup \set{
    (\vec{x}:\Theta) \vdash \MsX(\vec{x})~\Type}$, where $\MsX$ is a freely added formal symbol
  depending on the variables in $\Theta$.
  %
  Then, one has the pushout
  %
  \begin{equation*}
    \begin{tikzcd}
      \vvbr{\Ctx_\ell} \ar[r, hook] \ar[d, "\Theta"'] \ar[rd, phantom, "\ulcorner"{pos=1}]
      &
      \vvbr{\Ctx_\ell \vdash \Type} \ar[d, "\Theta.\MsX"]
      \\
      \vvbr{\McA} \ar[r, hook]
      &
      \vvbr{\McA^{(\vec{x}:\Theta).\MsX(\vec{x})}}
    \end{tikzcd} \in \CxlCat_\ITT
  \end{equation*}
  %
\end{lemma}
%
\begin{proof}
  %
  It is clear that $(\vec{x}:\Theta)~\Ctx$ is derivable using only axioms from
  $\coprod_{m<\ell}\McA_m^{(\vec{x}:\Theta).\MsX(\vec{x})} =
  \coprod_{m<\ell}\MsA_m$ because $(\vec{x}:\Theta) \in \vvbr{\MsA}$.
  %
  Suppose now that one has $\bC \in \CxlCat_\ITT$ along with maps
  %
  \begin{equation*}
    \begin{tikzcd}
      \vvbr{\Ctx_\ell} \ar[r, hook] \ar[d, hook, "\Theta"']
      &
      \vvbr{\Ctx_\ell \vdash \Type} \ar[d, "\Theta.\MsX"{description}]
      \ar[rdd, "G", bend left]
      \\
      \vvbr{\McA} \ar[r, hook]
      \ar[rrd, bend right=10, "F"']
      &
      \bC \ar[rd, dashed, "H"{description}]
      \\
      &
      &
      \bC
    \end{tikzcd} \in \CxlCat_\ITT
  \end{equation*}
  %
  Because $\vvbr{\Ctx_\ell \vdash \Type}$ is free, $G$ is entirely determined by
  $G\Ctx_\ell \in \ob_\ell\bC$ along with a type $G\Type \in \Ty{G\Ctx_\ell}$.
  %
  And commutativity says that $G\Ctx_\ell = F\Theta$.
  %
  Thus, one can define $H \colon \vvbr{\McA^{(\vec{x}:\Theta).\MsX}} \to \bC$ whose action on
  objects is defined by structural induction:
  %
  \begin{itemize}
    %
    \item $H() \coloneqq ()$
    %
    \item $H((\vec{y}:\Delta).\Pi(a:A(\vec{y}).B(\vec{y},a)))
    \coloneqq (\vec{y}:H\Delta).\Pi(a:HA(\vec{y})).HB(\vec{y},a)$
    if $\Delta \neq \Theta$.
    %
    \item $H((\vec{y}:\Delta).\Sigma(a:A(\vec{y}).B(\vec{y},a)))
    \coloneqq (\vec{y}:H\Delta).\Sigma(a:HA(\vec{y})).HB(\vec{y},a)$
    if $\Delta \neq \Theta$.
    %
    \item $H((\vec{y}:\Delta).(a_1~a_2:A(\vec{y})).\Id_{A(\vec{y})}(a_1,a_2))
    \coloneqq (\vec{y}:H\Delta).(a_1~a_2:HA(\vec{y})).\Id_{HA(\vec{y})}(a_1,a_2)$
    if $\Delta \neq \Theta$.
    %
    \item
    $H((\vec{x}:\Theta).\MsX(\vec{x})) \coloneqq
    (\vec{x}:F\Theta).G\MsX(\vec{x})$
    %
  \end{itemize}
  %
  and its action on maps is simply that of $F$.
  %
  Moreover, by structural induction on
  $\vvbr{\McA^{(\vec{x}:\Theta).\MsX}}$, this must be the unique such
  map $H$.
  %
\end{proof}

% \begin{lemma}
%   %
%   Suppose $\bC$ is syntactically presentable.
%   %
%   Then so is the pushout
%   %
%   \begin{equation*}
%     \begin{tikzcd}
%       \vvbr{\Ctx_\ell} \ar[r, hook] \ar[d, "\Theta"'] \ar[rd, phantom, "\ulcorner"{pos=1}]
%       &
%       \vvbr{\Ctx_\ell \vdash \Type} \ar[d]
%       \\
%       \bC \ar[r]
%       &
%       \bC \cup_{\vvbr{\Ctx_n}} \vvbr{\Ctx_n \vdash \Type}
%     \end{tikzcd}
%   \end{equation*}
%   %
% \end{lemma}
% %
% \begin{proof}
%   %
%   Let $\McA = \coprod_{n\in\bN}\McA_n$ be a syntactic presentation of $\bC$, so
%   that $\bC \cong \vvbr{\McA}$.
%   %
%   We claim that $\McA' \coloneqq \coprod_{n \in \bN}\McA'_n$ where
%   $\McA'_n \coloneqq \McA_n$ when $n \neq \ell$ and
%   $\McA'_\ell \coloneqq \McA_n \sqcup \set{\Theta \vdash \MsT~\Type}$
%   is such that $\vvbr{\McA'}$
%   %
%   Because $\Theta \in \bC$ and $\bC$ is syntactically presented by $\McA$, it is
%   derivable using only axioms in $\coprod_{m<n}\McA_m = \coprod_{m<n}\McA_n$.

%   Denote by $\vvbr{\McA'}$ and
%   %
% \end{proof}

\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "./main.tex"
%%% TeX-engine: xetex
%%% End:

